CM-PIE: Cross-modal perception for interactive-enhanced audio-visual video parsing

Audio-visual video parsing is the task of categorizing a video at the segment level with weak labels, and predicting them as audible or visible events. Recent methods for this task leverage the attention mechanism to capture the semantic correlations among the whole video across the audio-visual modalities. However, these approaches have overlooked the importance of individual segments within a video and the relationship among them, and tend to rely on a single modality when learning features. In this paper, we propose a novel interactive-enhanced cross-modal perception method~(CM-PIE), which can learn fine-grained features by applying a segment-based attention module. Furthermore, a cross-modal aggregation block is introduced to jointly optimize the semantic representation of audio and visual signals by enhancing inter-modal interactions. The experimental results show that our model offers improved parsing performance on the Look, Listen, and Parse dataset compared to other methods.

==> tables/sota.tex <==
\begin{table}[ht]
\begin{center}

\caption{\textbf{comparison with the state-of-the-art methods on the LLP dataset}.We calculate the event-level F-scores using a threshold of mIoU = 0.5. The overall Type@AV performance in the audio-visual scene is considered by averaging the evaluation results for audio, visual, and audio-visual events. Furthermore, Event@AV encompasses all audio and visual event categories for each individual sample.}

\scalebox{0.875}{

\begin{tabular}{cccccc}
% \hline
\midrule
\multicolumn{6}{c}{Segment-level}                \\ \hline
Method     & Audio & Visual & AV & Ty@AV & EV@AV \\ \hline 
AVE~\cite{tian2018audio} & 47.2 & 37.1 & {35.4} & {39.9} & 41.6 \\
AVSDN~\cite{lin2019dual} & 47.8 & 52.0 & {37.1} & {45.7} & 50.8 \\ 
HAN~\cite{tian2020unified} & {60.1} & {52.9} & 48.9 & 54 & 55.4 \\ 
CM-CS+HAN~\cite{chen2023cm} & {57.1} & {\textbf{57.6}} & 52.9 & 55.9 & 53.9 \\
MM-Pyramid~\cite{yu2022mm} & {60.9} & {54.4} & 51.8 & 55.1 & 57.6 \\  
Ours & {\textbf{61.7}} & {55.2} & 50.1 & 55.7 & 56.8 \\   
\hline
\multicolumn{6}{c}{Video-level}                   \\ 
\hline
AVE~\cite{tian2018audio} & 40.4 & 34.7 & {31.6} & {35.5} & 36.5 \\
AVSDN~\cite{lin2019dual} & 34.1 & 46.3 & {26.5} & {35.6} & 37.7 \\
HAN~\cite{tian2020unified} & 51.3 & 48.9 & {43} & {47.7} & 48 \\
CM-CS+HAN~\cite{chen2023cm} & {49.4} & {54.2} & 46.7 & 50.1 & 47.8 \\
MM-Pyramid~\cite{yu2022mm} & {52.7} & {50} & 44.4 & 49.9 & 50.5 \\ 
Ours & {\textbf{53.7}} & {51.3} & 43.6 & 49.5 &\textbf{51.3} \\
\hline
\end{tabular}

}

\vspace{-2.75em}
\label{cmp}
\end{center}
\end{table}

